SAS-Prompt: Large Language Models as Numerical Optimizers for Robot Self-Improvement

We demonstrate the ability of large language models (LLMs) to perform iterative self-improvement of robot policies. An important insight of this paper is that LLMs have a built-in ability to perform (stochastic) numerical optimization and that this property can be leveraged for explainable robot policy search. Based on this insight, we introduce the SAS Prompt (Summarize, Analyze, Synthesize) -- a single prompt that enables iterative learning and adaptation of robot behavior by combining the LLM's ability to retrieve, reason and optimize over previous robot traces in order to synthesize new, unseen behavior. Our approach can be regarded as an early example of a new family of explainable policy search methods that are entirely implemented within an LLM. We evaluate our approach both in simulation and on a real-robot table tennis task. Project website: sites.google.com/asu.edu/sas-llm/

==> table.tex <==
Example 0: (a:10.0, b:10.0, c:10.0, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
The ball travels with a moderate curve, reaching a peak height around the middle of the table and landing near the center on the opponent's side.
Example 1: (a:9.6, b:10.0, c:10.0, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
Similar trajectory to Example 0 but lands slightly further left and closer to the net on the opponent's side. The ball appears to have slightly less forward velocity.
Example 2: (a:9.8, b:10.0, c:10.0, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
Again, a similar trajectory with moderate curve and peak height, landing slightly right of center on the opponent's side. Forward velocity appears slightly higher than Example 0.
Example 3: (a:10.2, b:10.0, c:10.0, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
The ball exhibits a similar curve but lands slightly left of center on the opponent's side. The peak height seems slightly higher than in Example 0.
Example 4: (a:10.4, b:10.0, c:10.0, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
The trajectory has a more pronounced curve, landing further left on the opponent's side and closer to the net. The peak height seems comparable to Example 0.
Example 5: (a:10.0, b:9.6, c:10.0, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
The ball follows a straighter path with less curve and lands closer to the net on the opponent's side.
Example 6: (a:10.0, b:9.8, c:10.0, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
Similar to Example 5, the trajectory is straighter with less curve and lands near the center on the opponent's side.
Example 7: (a:10.0, b:10.2, c:10.0, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
The ball exhibits a more pronounced curve and lands further towards the right side of the opponent's half, closer to our objective.
Example 8: (a:10.0, b:10.4, c:10.0, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
This example results in a missed shot. The ball has a significant curve and lands outside the table on the left side.
Example 9: (a:10.0, b:10.0, c:9.6, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
The ball travels with a moderate curve, landing further back on the opponent's side compared to Example 0.
Example 10: (a:10.0, b:10.0, c:9.8, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
Similar trajectory to Example 9, but landing slightly closer to the net on the opponent's side.
Example 11: (a:10.0, b:10.0, c:10.2, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
The ball exhibits a more pronounced curve, landing slightly further right compared to Example 0.
Example 12: (a:10.0, b:10.0, c:10.4, d:10.0, e:10.0, f:10.0, g:10.0, h:10.0)
This example results in a missed shot with a significant curve, landing outside the table on the left side.
Example 13: (a:10.0, b:10.0, c:10.0, d:9.6, e:10.0, f:10.0, g:10.0, h:10.0)
The ball exhibits a pronounced curve, landing near the center on the opponent's side but with a higher peak height compared to Example 0.
Example 14: (a:10.0, b:10.0, c:10.0, d:9.8, e:10.0, f:10.0, g:10.0, h:10.0)
Similar trajectory to Example 13 but with a slightly lower peak height.
Example 15: (a:10.0, b:10.0, c:10.0, d:10.2, e:10.0, f:10.0, g:10.0, h:10.0)
The ball demonstrates a more pronounced curve and lands slightly right of center on the opponent's side.
Example 16: (a:10.0, b:10.0, c:10.0, d:10.4, e:10.0, f:10.0, g:10.0, h:10.0)
The ball travels with a significant curve, landing near the center of the opponent's side.
Example 17: (a:10.0, b:10.0, c:10.0, d:10.0, e:9.6, f:10.0, g:10.0, h:10.0)
The ball follows a straighter trajectory with less curve and lands slightly right of center on the opponent's side.
Example 18: (a:10.0, b:10.0, c:10.0, d:10.0, e:9.8, f:10.0, g:10.0, h:10.0)
Similar to Example 17, the ball travels with a straighter path and less curve, landing closer to the net on the opponent's side.
Example 19: (a:10.0, b:10.0, c:10.0, d:10.0, e:10.2, f:10.0, g:10.0, h:10.0)
The ball exhibits a more pronounced curve, landing left of center on the opponent's side and closer to the net.
Example 20: (a:10.0, b:10.0, c:10.0, d:10.0, e:10.4, f:10.0, g:10.0, h:10.0)
The ball shows a significant curve, landing closer to the right side of the opponent's half, but the trajectory seems somewhat unpredictable.
Example 21: (a:10.0, b:10.0, c:10.0, d:10.0, e:10.0, f:9.6, g:10.0, h:10.0)
The trajectory is straighter with less curve and lands closer to the net on the opponent's side.
Example 22: (a:10.0, b:10.0, c:10.0, d:10.0, e:10.0, f:9.8, g:10.0, h:10.0)
Similar to Example 21, the ball travels with a straighter path and less curve, landing near the center on the opponent's side.
Example 23: (a:10.0, b:10.0, c:10.0, d:10.0, e:10.0, f:10.2, g:10.0, h:10.0)
The ball demonstrates a more pronounced curve and lands slightly left of center on the opponent's side.
Step 1: Selecting Optimal Parameters
Based on the summaries and our objective to hit the ball to the far right side of the table, Examples 7 and 20 seem closest to fulfilling the objective. They both exhibit a pronounced curve and land on the right side of the opponent's half.
Step 2: Parameter Analysis
Parameter a: Increasing parameter a appears to slightly shift the landing position to the left and decrease forward velocity.
Parameter b: Increasing parameter b seems to create a more pronounced curve in the ball's trajectory.
Parameter c: Decreasing parameter c leads to a straighter ball trajectory with less curve.
Parameter d: Increasing parameter d creates a more pronounced curve and tends to push the ball towards the right side.
Parameter e: Increasing parameter e results in a straighter trajectory with less curve.
Parameter f: Decreasing parameter f leads to a straighter ball trajectory with less curve.
Parameters g & h: The provided examples don't offer sufficient variation in parameters g and h to determine their specific effects. More data with diverse values for these parameters would be needed for a proper analysis.

------ Interactive Querying -----

LLM Answer:  ## Step 1: Landing Position Summary

Here's a table summarizing the landing positions for each example, along with an analysis:

| Example | Landing X | Landing Y | Landing Z | On Opponent's Side | Close to Net |  Analysis |
|---|---|---|---|---|---|---| 
| 0 | -0.0177 | 0.3792 | 0.0050 | True | True | Very close to the net, slightly to the left of center, on the opponent's side. |
| 1 | 0.0321 | 0.8295 | -0.0123 | True | False |  Lands in the middle third of the opponent's side, further from the net. |
| 2 | 0.0138 | 0.6032 | -0.0243 | True | False | Lands closer to the middle of the opponent's side. |
| 3 | 0.1349 | 0.6391 | 0.0012 | True | False |  Lands further right on the opponent's side. |
| 4 | 0.0169 | 0.9172 | -0.0155 | True | False | Lands near the center, deep on the opponent's side. |
| 5 | 0.0231 | 1.1092 | -0.0004 | True | False | Lands near the center, very deep on the opponent's side, almost out. |
| 6 | 0.0241 | 1.2797 | -0.0252 | True | False | Lands near the center, very deep on the opponent's side, close to out. |
| 7 | -0.0040 | 1.1618 | 0.0033 | True | False |  Lands very close to the center, deep on the opponent's side. |
| 8 | 0.0979 | 1.1628 | -0.0091 | True | False | Lands on the right, deep on the opponent's side. |
| 9 | 0.2229 | 1.2401 | -0.0208 | True | False | Lands far right, very deep on the opponent's side, close to out. |
| 10 | 0.1110 | 1.2359 | 0.0136 | True | False | Lands on the right, very deep on the opponent's side, close to out. |
| 11 | -0.1073 | 1.1119 | -0.4000 | True | False | Lands on the left, deep on the opponent's side. |
| 12 | 0.1534 | 1.1071 | -0.0115 | True | False | Lands on the right, deep on the opponent's side. |
| 13 | 0.1707 | 1.0253 | -0.0151 | True | False | Lands on the right, deep on the opponent's side. |
| 14 | 0.0361 | 0.8046 | -0.0151 | True | False |  Lands near the center, on the opponent's side. |
| 15 | 0.2433 | 1.3173 | -0.0262 | True | False | Lands far right, very deep on the opponent's side, almost out. |
| 16 | 0.1403 | 1.2953 | -0.0206 | True | False |  Lands on the right, very deep on the opponent's side, close to out. |
| 17 | 0.0843 | 1.3418 | -0.0197 | True | False | Lands near the center, very deep on the opponent's side, almost out. |
| 18 | 0.0804 | 1.2972 | -0.0294 | True | False | Lands near the center, very deep on the opponent's side, close to out. |
| 19 | 0.0206 | 1.0632 | -0.0144 | True | False | Lands near the center, deep on the opponent's side. |
| 20 | 0.0951 | 1.2283 | 0.0041 | True | False | Lands on the right, very deep on the opponent's side, close to out. |
| 21 | 0.1856 | 1.2524 | -0.0135 | True | False | Lands on the right, very deep on the opponent's side, close to out. |
| 22 | 0.1145 | 0.6959 | 0.0148 | True | False |  Lands on the right, on the opponent's side. |
| 23 | 0.1346 | 1.2505 | 0.0008 | True | False | Lands on the right, very deep on the opponent's side, close to out. |
| 24 | 0.1665 | 0.6557 | -0.0180 | True | False |  Lands on the right, on the opponent's side. |
| 25 | -0.1264 | 0.4572 | -0.0043 | True | True | Lands close to the net on the left, on the opponent's side. |
| 26 | 0.2030 | 0.6139 | 0.0086 | True | False |  Lands on the right, on the opponent's side. |
| 27 | 0.0308 | 0.6364 | 0.0052 | True | False | Lands near the center, on the opponent's side. |
| 28 | 0.0951 | 0.9234 | 0.0063 | True | False | Lands on the right, deep on the opponent's side. |
| 29 | 0.1794 | 1.1504 | 0.0181 | True | False | Lands on the right, deep on the opponent's side. |
| 30 | 0.1955 | 1.2204 | -0.0106 | True | False | Lands on the right, very deep on the opponent's side, close to out. |
| 31 | 0.3676 | 0.5218 | -0.4018 | True | False | Lands far right on the opponent's side. |
| 32 | 0.1008 | 0.9453 | -0.0196 | True | False | Lands on the right, deep on the opponent's side. |
| 33 | 0.0895 | 1.2368 | -0.0180 | True | False | Lands near the center, very deep on the opponent's side, close to out. |
| 34 | -0.2949 | 0.8907 | -0.4000 | True | False | Lands far left on the opponent's side. |
| 35 | 0.2155 | 1.2713 | -0.0385 | True | False | Lands on the right, very deep on the opponent's side, close to out. |
| 36 | 0.1466 | 1.1857 | -0.0131 | True | False | Lands on the right, deep on the opponent's side. |
| 37 | 0.1065 | 1.2380 | 0.0016 | True | False | Lands on the right, very deep on the opponent's side, close to out. |
| 38 | -0.1996 | 0.0089 | 0.0325 | True | True |  Lands very close to the net on the left, on the opponent's side. |
| 39 | 0.1286 | 1.2564 | -0.0030 | True | False | Lands on the right, very deep on the opponent's side, close to out. |
| 40 | -0.0773 | 0.4572 | -0.0184 | True | True | Lands close to the net on the left, on the opponent's side. |
| 41 | 0.0423 | 1.2027 | -0.0026 | True | False | Lands near the center, very deep on the opponent's side, close to out. |
| 42 | 0.0570 | 1.1841 | -0.0097 | True | False | Lands near the center, deep on the opponent's side. |
| 43 | 0.0766 | 1.2568 | -0.0140 | True | False | Lands near the center, very deep on the opponent's side, close to out. |

## Step 2: Identifying the Closest Match

The objective is to hit the ball to the left. Focusing on examples where the ball lands on the table, we need to find the one with the most negative x-coordinate landing position.

**Example 34** has the most negative x-coordinate (-0.2949) making it the closest to the objective. 

## Step 3: Best Example

**Best example: 34**

**Best params: a:1.1 b:1.1 c:1.1 d:1.1 e:1.1 f:1.1 g:1.1 h:0.5** 



Total inference time:  97.54774761199951
Please provide your query to Gemini:
Hit it a little more in the other direction.
---------- Reusing Previous Answers for Speedup ---------------
LLM Answer:  The objective is to hit the ball a little more in the other direction, implying to the right, compared to the previous best example (Example 34). We need to find an example with a landing position on the table that is still on the left side (negative x) but closer to the center (x = 0) than Example 34's -0.2949.

Looking at the table, these examples land on the left side of the opponent's table:

* Example 0: x = -0.0177
* Example 7: x = -0.0040
* Example 11: x = -0.1073
* Example 25: x = -0.1264
* Example 34: x = -0.2949
* Example 38: x = -0.1996
* Example 40: x = -0.0773

Out of these, **Example 38** (x = -0.1996) is the closest to the center without crossing over to the positive x side. 

## Step 3: Best Example

**Best example: 38**

**Best params: a:1.1 b:1.1 c:1.1 d:1.1 e:1.1 f:0.7 g:1.1 h:0.5** 



Total inference time:  14.88242769241333
Please provide your query to Gemini:
Even more to the right.
---------- Reusing Previous Answers for Speedup ---------------
LLM Answer:  The objective is to hit the ball "even more to the right" than the previous best example (Example 38, landing at x = -0.1996). This means we are looking for an example that lands on the left side of the table but is even closer to the center (x = 0) than Example 38.

Looking at the table from our previous analysis, these candidates remain:

* Example 0: x = -0.0177
* Example 7: x = -0.0040
* Example 11: x = -0.1073
* Example 25: x = -0.1264
* Example 40: x = -0.0773 

Example 7 has the landing position closest to the center (x = -0.0040) while still remaining on the left side. 

## Step 3: Best Example

**Best example: 7**

**Best params: a:1.1 b:1.1 c:0.9 d:1.1 e:1.1 f:1.1 g:1.1 h:0.5** 



Total inference time:  23.770661115646362
Please provide your query to Gemini:
Even more to the right.
---------- Reusing Previous Answers for Speedup ---------------
LLM Answer:  Continuing from the previous analysis, the goal is to move the landing position "even more to the right" than Example 7 (landing at x = -0.0040). We are seeking an example that lands on the table, and since the instruction is to move further right, we need to cross over to the positive x values while staying as close to the center (x = 0) as possible.

The remaining candidates from the left side of the table are:

* Example 0: x = -0.0177

Looking at the examples that land on the right side of the table (positive x), and filtering for the ones closest to the center, we have:

* Example 1: x = 0.0321
* Example 2: x = 0.0138
* Example 4: x = 0.0169
* Example 5: x = 0.0231
* Example 6: x = 0.0241 
* Example 27: x = 0.0308

Comparing all the remaining candidates, **Example 2** with a landing position of x = 0.0138 is the closest to the center (x = 0) while being on the right side of the table. 

## Step 3: Best Example

**Best example: 2**

**Best params: a:1.1 b:1.1 c:0.7 d:1.1 e:1.1 f:1.1 g:1.1 h:0.5** 


